Bistable SMA-driven engine for pulse-jet locomotion in soft aquatic robots

This paper presents the design and experimental validation of a bio-inspired soft aquatic robot, the DilBot, which uses a bistable shape memory alloy-driven engine for pulse-jet locomotion. Drawing inspiration from the efficient swimming mechanisms of box jellyfish, the DilBot incorporates antagonistic shape memory alloy springs encapsulated in silicone insulation to achieve high-power propulsion. The innovative bistable mechanism allows continuous swimming cycles by storing and releasing energy in a controlled manner. Through free-swimming experiments and force characterization tests, we evaluated the DilBot's performance, achieving a peak speed of 158 mm/s and generating a maximum thrust of 5.59 N. This work demonstrates a novel approach to enhancing the efficiency of shape memory alloy actuators in aquatic environments. It presents a promising pathway for future applications in underwater environmental monitoring using robotic swarms.

==> text/notes.tex <==







TO DO LIST:

    Figures:
        - Mechanical Overview
            - Split into two figures                      [DONE ]
            - adjust energy curve to be hump  [DONE]
            - remove a) and b)                             [DONE]
            - retitle SMA springs                          [DONE]
            - ensure figures have same height              [DONE]

        - Bistability
            - Design hump                                  [DONE]
            - Label Important Regions                      [DONE]
        
        - Thrust Force Experimental Set Up
            - 

        - Flow Visualization Lab Set Up
            - 

        - Free Swim
            - Shade up vs downstroke instead of dots,       [DONE]
            remove from legend and label                    []
            - Enlarge axis label and text                   []
            - remove box from legend                        [DONE]
            - color axis                                    [DONE]
            - split image                                   []

        - Thrust Force
            - enlarge text/labels
            - remove legend box.
            - Change time to ms instead of decimal seconds
            - indicate snap through point
            - annotate period: expansion, contraction, glide
    
        FLOW VIZ
            - Choose Frames
            - High Contrast
            - Correct Timing



ORDER OF OPERATIONS:
    1. Rewrite Methods and Address Comments [DONE]
    2. Remake Figures                       [DONE]
    3. FLOW VIS
    4. Add to Results and Discussion        []
    5. Assemble DARS Demonstration Items    []
    


TMO MORNING:
    - STANDARDIZE
    - FINAL FIGURE CHECK
    - FINALIZE RESULTS
        - FLOW VIZ



    - DARS
        - 

    

